Engineering AI Judge Systems

AI judge systems are designed to automatically evaluate Foundation Model-powered software (i.e., FMware). Due to the intrinsic dynamic and stochastic nature of FMware, the development of AI judge systems requires a unique engineering life cycle and presents new challenges. In this paper, we discuss the challenges based on our industrial experiences in developing AI judge systems for FMware. These challenges lead to substantial time consumption, cost and inaccurate judgments. We propose a framework that tackles the challenges with the goal of improving the productivity of developing high-quality AI judge systems. Finally, we evaluate our framework with a case study on judging a commit message generation FMware. The accuracy of the judgments made by the AI judge system developed with our framework outperforms those made by the AI judge system that is developed without our framework by up to 6.2%, with a significant reduction in development effort.

==> abstract.tex <==
\begin{abstract}
% Recent emergence of building foundation model-based (FM-based) applications 


\xjudgesystems are designed to automatically evaluate Foundation Model-powered software (i.e., \xapp). Due to the intrinsic dynamic and stochastic nature of \xapp, the development of \xjudgesystems requires a unique engineering life cycle and presents new challenges. In this paper, we discuss the challenges based on our industrial experiences in developing \xjudgesystems for \xapp. These challenges lead to substantial time consumption, cost and inaccurate judgments. We propose a framework that tackles the challenges with the goal of improving the productivity of developing high-quality \xjudgesystems. 
Finally, we evaluate our framework with a case study on judging a commit message generation FMware. %, that is important for program comprehension and the maintenance of a software project. 
The accuracy of the judgments made by the \xjudgesystem developed with our framework outperforms those made by the \xjudgesystem that is developed without our framework by up to 6.2\%, with a significant reduction in development effort.
\end{abstract}
